An Extensive Evaluation of the Internet's Open Proxies

Open proxies forward traffic on behalf of any Internet user. Listed on open proxy aggregator sites, they are often used to bypass geographic region restrictions or circumvent censorship. Open proxies sometimes also provide a weak form of anonymity by concealing the requestor's IP address. To better understand their behavior and performance, we conducted a comprehensive study of open proxies, encompassing more than 107,000 listed open proxies and 13M proxy requests over a 50 day period. While previous studies have focused on malicious open proxies' manipulation of HTML content to insert/modify ads, we provide a more broad study that examines the availability, success rates, diversity, and also (mis)behavior of proxies. Our results show that listed open proxies suffer poor availability--more than 92% of open proxies that appear on aggregator sites are unresponsive to proxy requests. Much more troubling, we find numerous examples of malicious open proxies in which HTML content is manipulated to mine cryptocurrency (that is, cryptojacking). We additionally detect TLS man-in-the-middle (MitM) attacks, and discover numerous instances in which binaries fetched through proxies were modified to include remote access trojans and other forms of malware. As a point of comparison, we conduct and discuss a similar measurement study of the behavior of Tor exit relays. We find no instances in which Tor relays performed TLS MitM or manipulated content, suggesting that Tor offers a far more reliable and safe form of proxied communication.

==> sections/results-table.tex <==
\begin{table}
\centering
\begin{small}
\begin{tabular}{p{1.5in}|p{0.60in}|p{0.75in}}

{\bf Attack Type} & {\bf Observed?}  &  {\bf \% Proxies}\\ \toprule

HTTP and Javascript Manipulation            & Yes       & 1.23\% (15/1220)  \\
HTTP Header Manipulation                    & Yes       & 55\% (650/1182)    \\
Shell Script Manipulation                   & No        & --                \\
EXE Manipulation                            & Yes       & 0.51\% (6/1163)   \\
SSL Stripping                               & No        & --                \\
SSL Certificate Manipulation                & No        & --                \\ \hline

\end{tabular}
\end{small}
\caption{Summary of exhibited malicious behavior by open proxies.}
\label{tbl:bad-proxies-summary}
\end{table}


==> tables/html/suspicious.tex <==

\begin{table}[h]
\centering
\begin{small}
\begin{tabular}{llr}
\toprule
    {\bf Label} & {\bf Malicious} & {\bf Count} \\
\midrule
Equivalent & N & 7 \\
Misconfiguration & N & 33 \\
No Content & N & 4 \\ 
Truncated & N & 2 \\
Unauthorized & N & 89\\
Ad Injection & Y & 20\\
Cryptojacking & Y & 5\\
Original + Ad Injection & Y & 2 \\
Potential Eavesdropping & Y & 1 \\
Unlabeled & May Be & 6 \\
\midrule
Total &  & 169 \\
\bottomrule
\end{tabular}
\end{small}
\caption{Classification of modified html on 2018-05-07}
\label{tbl:html-suspicious-category}
\end{table}

